Individual Heterogeneity and Cultural Attitudes in Credence Goods Provision

I study the heterogeneity of credence goods provision in taxi drivers taking detours in New York City. First, I document that there is significant detouring on average by drivers. Second, there is significant heterogeneity in cheating across individuals, yet each individual's propensity to take detours is stable: drivers who detour almost always detour, while those who do not detour almost never do. Drivers who take longer detours on each trip also take such trips more often. Third, cultural attitudes plausibly explain some of this heterogeneity in behavior across individuals.

==> plots/GPS-coordinates.tex <==

\begin{table}[!htbp]
\centering
\caption{Latitudes and Longitudes}
\label{GPS-coordinates}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                             & \multicolumn{2}{c|}{Latitude} & \multicolumn{2}{c|}{Longitude} \\ \hline
\begin{tabular}[c]{@{}c@{}}Area of\\   Interest\end{tabular} & Minimum       & Maximum       & Minimum        & Maximum       \\ \hline
Midtown East                                                 & 40.748132     & 40.762696     & -73.979109     & -73.962973    \\ \hline
LaGuardia Airport                                            & 40.766332     & 40.777488     & -73.882291     & -73.860748    \\ \hline
JFK Airport                                                  & 40.628159     & 40.668073     & -73.828243     & -73.761891    \\ \hline
\end{tabular}
\end{table}

This table reports the latitude and longitude ranges of the three main areas of interest in the paper: midtown east, LaGuardia airport, and JFK airport. Trips to each of the areas are defined as trips whose recorded drop-off GPS coordinates fall within the drop-off latitude and longitude ranges. Trips from each of the areas are defined as trips whose recorded pick-up GPS coordinates fall within the pick-up latitude and longitude ranges.

==> plots/cultural_regs.tex <==
\begin{table}[H]
\caption{Cultural Attitudes and Detour Distances}
\label{cultural_regs}
\begin{tabular}{lcccccc}
               & \multicolumn{2}{c}{LGA Detour Distance} & LGA             & \multicolumn{2}{c}{JFK Detour Distance} & JFK             \\\hline
VARIABLES      & In-Sample         & Google Maps         & Number of Trips & In-Sample         & Google Maps         & Number of Trips \\
CPI Score 2013 & 0.0265***         & 0.0147***           & 0.295***        & -0.00529          & -0.0118*            & -0.430***       \\
               & (0.00541)         & (0.00548)           & (0.0651)        & (0.00803)         & (0.00702)           & (0.0748)        \\
               &                   &                     &                 &                   &                     &                 \\
Constant       & -0.106***         & 0.234***            & 12.27***        & 0.0497*           & 0.237***            & 5.233***        \\
               & (0.0194)          & (0.0196)            & (0.246)         & (0.0293)          & (0.0261)            & (0.257)         \\
               &                   &                     &                 &                   &                     &                 \\
Observations   & 22,503            & 22,824              & 22,824          & 16,149            & 17,442              & 17,442          \\
R-squared      & 0.001             & 0.000               & 0.001           & 0.000             & 0.000               & 0.003           \\\hline
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}Robust\\   standard errors in parentheses\end{tabular}}                                  \\
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}***\\   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1\end{tabular}}          
                                    
\end{tabular}
\end{table}



==> plots/cultural_regs_1998.tex <==
\begin{table}[H]
\caption{Cultural Attitudes and Detour Distances (1998 CPI)}
\label{cultural_regs_1998}
\begin{tabular}{lcccccc}
               & \multicolumn{2}{c}{LGA Detour Distance} & LGA             & \multicolumn{2}{c}{JFK Detour Distance} & JFK             \\\hline
VARIABLES      & In-Sample         & Google Maps         & Number of Trips & In-Sample         & Google Maps         & Number of Trips \\
CPI Score 2013 & 0.0193***         & 0.0165***           & 0.248***        & -0.00901          & -0.0182***          & -0.111          \\
               & (0.00548)         & (0.00555)           & (0.0649)        & (0.00795)         & (0.00691)           & (0.0769)        \\
               &                   &                     &                 &                   &                     &                 \\
Constant       & -0.167***         & 0.214***            & 11.49***        & 0.0354            & 0.206***            & 6.771***        \\
               & (0.0197)          & (0.0200)            & (0.251)         & (0.0286)          & (0.0254)            & (0.269)         \\
               &                   &                     &                 &                   &                     &                 \\
Observations   & 18,102            & 18,371              & 18,371          & 13,237            & 14,269              & 14,269          \\
R-squared      & 0.001             & 0.001               & 0.001           & 0.000             & 0.000               & 0.000           \\\hline
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}Robust\\   standard errors in parentheses\end{tabular}}                                  \\
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}***\\   p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1\end{tabular}}          

\end{tabular}
\end{table}

==> plots/cultural_regs_unweighted.tex <==
\begin{table}[H]
\caption{Cultural Attitudes and Detour Distances (Unweighted)}
\label{cultural_regs_unweighted}
\begin{tabular}{lcccccc}
               & \multicolumn{2}{c}{LGA Detour Distance} & LGA             & \multicolumn{2}{c}{JFK Detour Distance} & JFK             \\
VARIABLES      & In-Sample         & Google Maps         & Number of Trips & In-Sample         & Google Maps         & Number of Trips \\ \hline
CPI Score 2013 & 0.0372***         & 0.0242***           & 0.305***        & -0.00832          & -0.0120*            & -0.495***       \\
               & (0.00498)         & (0.00505)           & (0.0600)        & (0.00747)         & (0.00661)           & (0.0658)        \\
               &                   &                     &                 &                   &                     &                 \\
Constant       & 0.182***          & 0.552***            & 12.33***        & 0.0385            & 0.235***            & 4.965***        \\
               & (0.0240)          & (0.0231)            & (0.234)         & (0.0281)          & (0.0252)            & (0.229)         \\
               &                   &                     &                 &                   &                     &                 \\
Observations   & 22,503            & 22,824              & 22,824          & 16,149            & 17,442              & 17,442          \\
R-squared      & 0.003             & 0.001               & 0.001           & 0.000             & 0.000               & 0.004           \\ \hline
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}Robust standard errors in parentheses\end{tabular}}                                  \\
\multicolumn{7}{l}{\begin{tabular}[c]{@{}l@{}}*** p\textless{}0.01, ** p\textless{}0.05, * p\textless{}0.1\end{tabular}}          
\end{tabular}
\end{table}

==> plots/demographics-questions.tex <==
\begin{table}[H]
\centering
\caption{Survey Questions}
\label{demographics-questions}
\begin{tabular}{|c|c|c|}
\hline
Survey                                                                             & Question                                                                                                                                                                                                                                                                                                      & Response Format                                                                                                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Transparency \\ International\end{tabular}              & \begin{tabular}[c]{@{}c@{}}Corruption Perception\\  Index 1998\end{tabular}                                                                                                                                                                                                                                   & \begin{tabular}[c]{@{}c@{}}Scale from -10 to \\ 0, where -10 means\\  least corrupt and 0 \\ means most corrupt.\end{tabular}                                            \\ \hline
\begin{tabular}[c]{@{}c@{}}Pew Research \\ Global Attitudes\\  Survey\end{tabular} & \begin{tabular}[c]{@{}c@{}}Most People in \\ Society are\\   Trustworthy?\end{tabular}                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}c@{}}Percent of respondents \\ who disagree with\\  the statement minus \\ percent of respondents\\  who agree with \\ the statement.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}World Values\\  survey\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Could you tell me \\ for each whether\\ you trust people from \\ this group completely,\\  somewhat, not very\\  much or not at all? \\   V105 People you meet \\ for the first time\\   V106 People of \\ another religion\\   V107 People of \\ another nationality\end{tabular} & \begin{tabular}[c]{@{}c@{}}Scale from 1 to 4,\\  with 1 meaning \\ “trust completely” \\ and 4 meaning \\ “do not trust at all”.\end{tabular}                            \\ \hline
\begin{tabular}[c]{@{}c@{}}World Values\\  survey\end{tabular}                     & \begin{tabular}[c]{@{}c@{}}Please tell me for each\\  of the following actions\\  whether you think \\ it can always be \\ justified, never be\\   justified, or something\\  in between \\   V200 Stealing property\end{tabular}                                                                             & \begin{tabular}[c]{@{}c@{}}Scale from 1 to 10, \\ with 1 meaning\\   “never justifiable” \\ and 10 meaning \\ “always justifiable”.\end{tabular}                         \\ \hline
\end{tabular}
\end{table}

This table reports the survey questions used in the demographics analysis in section 7. The table reports the survey source, the wording of the question in English that was asked, and the response format of how answers to survey questions were collected. The response formats to the Transparency International and Pew Research Global Attitudes Survey have been transformed so that a greater numerical score corresponds to a notion of higher corruption or lower trust.


==> plots/demographics-results.tex <==
\begin{table}[H]
\centering
\caption{Demographics Results}
\label{demographics-results}
\begin{tabular}{|c|c|c|c|c|}
\hline
                             & LGA                                                                  & LGA                                                         & JFK                                                                  & JFK                                                         \\ \hline
Ethnicity                    & \begin{tabular}[c]{@{}c@{}}Avg. Detour \\ Dist. (miles)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Num. \\ Trips\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg. Detour \\ Dist. (miles)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Num. \\ Trips\end{tabular} \\ \hline
African,EastAfrican          & -0.20***                                                             & 1208                                                        &                                                                      &                                                             \\ \hline
African,WestAfrican          & -0.10***                                                             & 7405                                                        & 0.11***                                                              & 3069                                                        \\ \hline
CelticEnglish                & -0.13***                                                             & 15827                                                       & 0.00                                                                 & 9330                                                        \\ \hline
EastAsian,Chinese            & -0.23***                                                             & 3277                                                        & 0.05                                                                 & 1352                                                        \\ \hline
EastAsian,Malay,Indonesia    & -0.06***                                                             & 4241                                                        & -0.12***                                                             & 1864                                                        \\ \hline
European,French(Haitian)     & -0.33***                                                             & 31525                                                       & 0.04***                                                              & 23938                                                       \\ \hline
European,German              & -0.06                                                                & 1311                                                        &                                                                      &                                                             \\ \hline
European,Russian             & 0.27***                                                              & 2716                                                        & -0.22***                                                             & 2476                                                        \\ \hline
Greek                        & 0.29***                                                              & 2177                                                        &                                                                      &                                                             \\ \hline
Hispanic,Portuguese          & -0.11***                                                             & 1360                                                        &                                                                      &                                                             \\ \hline
Hispanic,Spanish             & 0.07***                                                              & 13345                                                       & 0.03                                                                 & 3740                                                        \\ \hline
Muslim,Nubian                & -0.09***                                                             & 13406                                                       & 0.01                                                                 & 4432                                                        \\ \hline
Muslim,Pakistanis,Bangladesh & 0.14***                                                              & 53068                                                       & 0.06***                                                              & 11707                                                       \\ \hline
Muslim,Pakistanis,Pakistan   & 0.08***                                                              & 24964                                                       & -0.03***                                                             & 10871                                                       \\ \hline
Muslim,Persian               & 0.09***                                                              & 7531                                                        & 0.06**                                                               & 2824                                                        \\ \hline
SouthAsian                   & 0.11***                                                              & 63315                                                       & -0.04***                                                             & 31908                                                       \\ \hline
\end{tabular}
\end{table}

*** p<0.01, ** p<0.05, * p<0.1

The table above reports the average detour distances and numbers of LaGuardia-to-midtown east and JFK-to-midtown east trips made by drivers tabulated by ethnicity. Only ethnicities with at least 1,000 trips from the specified airport have the average detour distance and number of trips reported for that ethnicity for that airport. The methodology for computing average detour distances and classifying ethnicity is in section 7.


==> plots/demographics-simulation.tex <==
\begin{table}[H]
\centering
\caption{Simulation of Average Number of Ethnicities Represented Per Medallion}
\label{demographics-simulation}
\begin{tabular}{|l|l|}
\hline
Mean      & 3.22029 \\ \hline
Std. Dev. & 0.00491 \\ \hline
Minimum   & 3.20408 \\ \hline
25\%      & 3.217   \\ \hline
50\%      & 3.22031 \\ \hline
75\%      & 3.22354 \\ \hline
Maximum   & 3.23574 \\ \hline
\end{tabular}
\end{table}

The table reports the results of the demographics simulation in section 7. The summary statistics are of the average number of ethnicities represented per medallion in each simulation.

==> plots/experience-JFK.tex <==
\begin{table}[H]
\centering
\caption{JFK Frequency of Visits}
\label{experience-JFK}
\begin{tabular}{|c|c|c|}
\hline
                                                                              & (1)           & (2)             \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variable:\end{tabular}               & Trip Distance & Detour Distance \\ \hline
                                                                              &               &                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Number\\   of JFK Trips Driven\end{tabular}        & 0.000495      & 0.000718        \\ \hline
                                                                              & (0.000488)    & (0.000475)      \\ \hline
Constant                                                                      & 17.58***      & 0.214***        \\ \hline
                                                                              & (0.0101)      & (0.00987)       \\ \hline
                                                                              &               &                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Time and Destination \\ Fixed Effects\end{tabular} & 137,470       & 137,470         \\ \hline
                                                                              & 0.118         & 0.192           \\ \hline
Observations                                                                  & 296,748       & 296,748         \\ \hline
R-squared                                                                     & 0.191         & 0.195           \\ \hline
\multicolumn{3}{|l|}{Standard errors in parentheses}                                                            \\ \hline
\multicolumn{3}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                    \\ \hline
\end{tabular}
\end{table}

==> plots/experience-LGA.tex <==
\begin{table}[H]
\centering
\caption{LaGuardia Frequency of Visits}
\label{experience-LGA}
\begin{tabular}{|c|c|c|}
\hline
                                                                              & (1)           & (2)             \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variable:\end{tabular}               & Trip Distance & Detour Distance \\ \hline
                                                                              &               &                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Number\\   of LaGuardia Trips Driven\end{tabular}  & 0.0100***     & 0.0101***       \\ \hline
                                                                              & (0.000602)    & (0.000560)      \\ \hline
Constant                                                                      & 9.593***      & 0.128***        \\ \hline
                                                                              & (0.0140)      & (0.0132)        \\ \hline
                                                                              &               &                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Time and Destination \\ Fixed Effects\end{tabular} & Yes           & Yes             \\ \hline
                                                                              &               &                 \\ \hline
Observations                                                                  & 296,748       & 296,748         \\ \hline
R-squared                                                                     & 0.191         & 0.195           \\ \hline
\multicolumn{3}{|l|}{Standard errors in parentheses}                                                            \\ \hline
\multicolumn{3}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                    \\ \hline
\end{tabular}
\end{table}

==> plots/intra-medallion.tex <==
\begin{table}[H]
\centering
\caption{LaGuardia Intra-Medallion Detour Distance Regression}
\label{intra-medallion}
\begin{tabular}{|c|c|}
\hline
                                                                              & (1)                  \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variable:\end{tabular}               & Avg. Detour Distance \\ \hline
                                                                              &                      \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg. Detour Dist. \\ Of Other Drivers\end{tabular} & 0.147749***          \\ \hline
                                                                              & (0.008481)           \\ \hline
Constant                                                                      & 0.130365***          \\ \hline
                                                                              & (0.005629)           \\ \hline
                                                                              &                      \\ \hline
Observations                                                                  & 55948                \\ \hline
R-squared                                                                     & 0.01                 \\ \hline
\multicolumn{2}{|c|}{Standard errors in parentheses}                                                 \\ \hline
\multicolumn{2}{|c|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                         \\ \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{JFK Intra-Medallion Detour Distance Regression}
\label{my-label}
\begin{tabular}{|c|c|}
\hline
                                                                              & (1)                  \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variable:\end{tabular}               & Avg. Detour Distance \\ \hline
                                                                              &                      \\ \hline
\begin{tabular}[c]{@{}c@{}}Avg. Detour Dist. \\ Of Other Drivers\end{tabular} & 0.047153***          \\ \hline
                                                                              & (0.008677)           \\ \hline
Constant                                                                      & 0.231551***          \\ \hline
                                                                              & (0.008219)           \\ \hline
                                                                              &                      \\ \hline
Observations                                                                  & 32256                \\ \hline
R-squared                                                                     & 0.00                 \\ \hline
\multicolumn{2}{|c|}{Standard errors in parentheses}                                                 \\ \hline
\multicolumn{2}{|c|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                         \\ \hline
\end{tabular}
\end{table}

The tables report the regression of average detour distances of a taxi driver on the average detour distances of other drivers who share a medallion with the given driver for trips from each airport. The distances are measured in miles. Each observation is an individual driver. The average detour distances in the dependent and independent variables are calculated from the same airport. For example, in the JFK regression, both variables are calculated using only JFK trips. In the LaGuardia regression, both variables are calculated using only LaGuardia trips.

==> plots/jfk-time-regressions-match-samples.tex <==
\begin{table}[H]
\centering
\caption{JFK Time Regressions - Match Samples}
\label{jfk-time-regressions-match-samples}
\begin{tabular}{|c|c|c|c|}
\hline
                                                               & (1)       & (2)                                                                     & (3)                                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent \\ variable:\end{tabular} & Trip Time & \begin{tabular}[c]{@{}c@{}}Time Discrepancy Google \\ Maps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time Discrepancy \\ In-Sample\end{tabular} \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
\begin{tabular}[c]{@{}c@{}}Detour \\ Distance\end{tabular}     & 1.554***  & 1.711***                                                                & 1.560***                                                              \\ \hline
                                                               & (0.0482)  & (0.0483)                                                                & (0.0493)                                                              \\ \hline
Constant                                                       & 40.19***  & 3.379***                                                                & -0.368***                                                             \\ \hline
                                                               & (0.0451)  & (0.0437)                                                                & (0.0462)                                                              \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Time FEs                                                       & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
Destination FEs                                                & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Observations                                                   & 132,852   & 132,852                                                                 & 132,852                                                               \\ \hline
R-squared                                                      & 0.478     & 0.466                                                                   & 0.035                                                                 \\ \hline
\multicolumn{4}{|l|}{Standard errors in parentheses}                                                                                                                                                                         \\ \hline
\multicolumn{4}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                                                                                                                                 \\ \hline
\end{tabular}
\end{table}

==> plots/jfk-time-regressions.tex <==
\begin{table}[H]
\centering
\caption{JFK Time Regressions}
\label{jfk-time-regressions}
\begin{tabular}{|c|c|c|c|}
\hline
                                                               & (1)       & (2)                                                                     & (3)                                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent \\ variable:\end{tabular} & Trip Time & \begin{tabular}[c]{@{}c@{}}Time Discrepancy Google \\ Maps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time Discrepancy \\ In-Sample\end{tabular} \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
\begin{tabular}[c]{@{}c@{}}Detour \\ Distance\end{tabular}     & 1.540***  & 1.695***                                                                & 1.560***                                                              \\ \hline
                                                               & (0.0495)  & (0.0497)                                                                & (0.0493)                                                              \\ \hline
Constant                                                       & 39.97***  & 3.148***                                                                & -0.368***                                                             \\ \hline
                                                               & (0.0449)  & (0.0436)                                                                & (0.0462)                                                              \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Time FEs                                                       & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
Destination FEs                                                & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Observations                                                   & 137,470   & 137,470                                                                 & 132,852                                                               \\ \hline
R-squared                                                      & 0.481     & 0.470                                                                   & 0.035                                                                 \\ \hline
\multicolumn{4}{|l|}{Standard errors in parentheses}                                                                                                                                                                         \\ \hline
\multicolumn{4}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                                                                                                                                 \\ \hline
\end{tabular}
\end{table}

==> plots/lga-jfk-table.tex <==
\begin{table}[H]
\centering
\caption{Detour Distances of LaGuardia and JFK Trips}
\label{lga-jfk-table}
\begin{tabular}{|c|c|c|c|c|}
\hline
                        &                            & LaGuardia trips & JFK trips & LGA-JFK \\ \hline
Average detour distance & (miles)                    & 0.42            & 0.23      & +0.19   \\ \hline
                        & (\% of trip dist.)                       & 5.6\%           & 1.5\%     & +4.1\%  \\ \hline
Percent of trips with   & \textgreater1-mile detours & 32\%            & 11\%      & +21\%   \\ \hline
                        & \textgreater2-mile detours & 14\%            & 8\%       & +6\%    \\ \hline
Percent of trips with   & \textgreater10\% detours   & 32\%            & 8\%       & +24\%   \\ \hline
                        & \textgreater20\% detours   & 18\%            & 5\%       & +13\%   \\ \hline
\end{tabular}
\end{table}

==> plots/lga-left-tail.tex <==
\begin{table}[H]
\centering
\caption{Left Tail in LaGuardia Detour Distances Histogram}
\label{lga-left-tail}
\begin{tabular}{cccc}

           & Detour Distance     & Percentage of Trips with no Tolls & Average Toll Amount \\ \hline
All        &                     & 10.4\%                            & \$4.71              \\ 
Left Tail  & \textless -1 Mile   & 35.3\%                            & \$3.41              \\ 
Right Tail & \textgreater 1 Mile & 4.8\%                             & \$5.01              \\ \hline
\end{tabular}
\end{table}

This table reports the percent of LaGuardia to Manhattan trips that had no tolls by their detour distance. The percent of trips with no tolls and average toll amounts are repoted for each sub-sample of trips. The left tail corresponds to trips with a detour distance of <-1 mile. The right tail corresponds to trips with a detour distance of >-1 mile.

==> plots/lga-time-regressions-match-samples.tex <==
\begin{table}[]
\centering
\caption{LaGuardia Time Regressions - Match Samples}
\label{lga-time-regressions-match-samples}
\begin{tabular}{|c|c|c|c|}
\hline
                                                               & (1)       & (2)                                                                     & (3)                                                                   \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent \\ variable:\end{tabular} & Trip Time & \begin{tabular}[c]{@{}c@{}}Time Discrepancy Google \\ Maps\end{tabular} & \begin{tabular}[c]{@{}c@{}}Time Discrepancy \\ In-Sample\end{tabular} \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
\begin{tabular}[c]{@{}c@{}}Detour \\ Distance\end{tabular}     & 0.382***  & 0.435***                                                                & 0.376***                                                              \\ \hline
                                                               & (0.0187)  & (0.0183)                                                                & (0.0188)                                                              \\ \hline
Constant                                                       & 26.73***  & 2.909***                                                                & -0.159***                                                             \\ \hline
                                                               & (0.0221)  & (0.0213)                                                                & (0.0222)                                                              \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Time FEs                                                       & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
Destination FEs                                                & Yes       & Yes                                                                     & Yes                                                                   \\ \hline
                                                               &           &                                                                         &                                                                       \\ \hline
Observations                                                   & 294,378   & 294,378                                                                 & 294,378                                                               \\ \hline
R-squared                                                      & 0.401     & 0.337                                                                   & 0.004                                                                 \\ \hline
\multicolumn{4}{|l|}{Standard errors in parentheses}                                                                                                                                                                         \\ \hline
\multicolumn{4}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                                                                                                                                 \\ \hline
\end{tabular}
\end{table}

==> plots/lga-variance.tex <==
\begin{table}[H]
\centering
\caption{LaGuardia Trip Time Variance}
\label{lga-variance}
\begin{tabular}{cccc}

LGA                                                                         & \begin{tabular}[c]{@{}c@{}}Detour distance \\ \textless -1-mile\end{tabular} & \begin{tabular}[c]{@{}c@{}}Detour distance between\\  -1 and 1 mile\end{tabular} & \begin{tabular}[c]{@{}c@{}}Detour distance\\  \textgreater 1-mile\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Standard deviation \\ of trip times\end{tabular} & 8.03                                                                         & 7.34                                                                             & 7.81                                                                           \\ \hline
\end{tabular}
\end{table}

This table reports the standard deviations of LaGuardia to Manhattan trip times by detour distances. The measure of trip times used here is time discrepancy in-sample. For example, the standard deviation of trip times of trips with detour distance between -1 and 1 mile is 7.34. The measurement unit of trips times is minutes.

==> plots/persistence-predictability-jfk.tex <==
\begin{table}[]
\centering
\caption{Trip Distance Residual Predictability - JFK Trips}
\label{persistence-predictability-jfk}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                                                      & (1)                                                                      & (2)                                                                      & (3)                                                                      & (4)                                                                      \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variables:\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}JFK Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}JFK Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}LGA Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}LGA Trip \\ Distance \\ Residual\end{tabular} \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Driver JFK Trip \\ Distance \\ Residuals (H1)\end{tabular} & 0.445***                                                                 & 0.427***                                                                 & 0.0683***                                                                & 0.0507***                                                                \\ \hline
                                                                                      & (0.0104)                                                                 & (0.0166)                                                                 & (0.00334)                                                                & (0.00784)                                                                \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Google\\   Maps Distance\end{tabular}                      &                                                                          & -0.00850                                                                 &                                                                          & 0.00570                                                                  \\ \hline
                                                                                      &                                                                          & (0.00889)                                                                &                                                                          & (0.00555)                                                                \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
Constant                                                                              & -0.00225                                                                 & 0.145                                                                    & -0.0122***                                                               & -0.0649                                                                  \\ \hline
                                                                                      & (0.00497)                                                                & (0.155)                                                                  & (0.00394)                                                                & (0.0538)                                                                 \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Time and \\ Destination \\ Fixed Effects\end{tabular}      & No                                                                       & Yes                                                                      & No                                                                       & Yes                                                                      \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
Observations                                                                          & 62,140                                                                   & 62,140                                                                   & 97,247                                                                   & 97,247                                                                   \\ \hline
R-squared                                                                             & 0.073                                                                    & 0.183                                                                    & 0.004                                                                    & 0.128                                                                    \\ \hline
\multicolumn{5}{|l|}{Robust standard errors in parentheses}                                                                                                                                                                                                                                                                                                                                       \\ \hline
\multicolumn{5}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                                                                                                                                                                                                                                                                                                      \\ \hline
\end{tabular}
\end{table}

==> plots/persistence-predictability-lga.tex <==
\begin{table}[H]
\centering
\caption{Trip Distance Residual Predictability - LaGuardia Trips}
\label{persistence-predictability-lga}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                                                                      & (1)                                                                      & (2)                                                                      & (3)                                                                      & (4)                                                                      \\ \hline
\begin{tabular}[c]{@{}c@{}}Dependent\\   variables:\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}LGA Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}LGA Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}JFK Trip \\ Distance \\ Residual\end{tabular} & \begin{tabular}[c]{@{}c@{}}JFK Trip \\ Distance \\ Residual\end{tabular} \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Driver LGA Trip \\ Distance \\ Residuals (H1)\end{tabular} & 0.775***                                                                 & 0.747***                                                                 & 0.0541***                                                                & 0.0423***                                                                \\ \hline
                                                                                      & (0.00374)                                                                & (0.00720)                                                                & (0.00603)                                                                & (0.0100)                                                                 \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Google\\   Maps Distance\end{tabular}                      &                                                                          & -0.0494***                                                               &                                                                          & 0.0132                                                                   \\ \hline
                                                                                      &                                                                          & (0.00355)                                                                &                                                                          & (0.0102)                                                                 \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
Constant                                                                              & -0.00191                                                                 & 0.466***                                                                 & 0.0213***                                                                & -0.210                                                                   \\ \hline
                                                                                      & (0.00274)                                                                & (0.0341)                                                                 & (0.00569)                                                                & (0.177)                                                                  \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
\begin{tabular}[c]{@{}c@{}}Time and \\ Destination \\ Fixed Effects\end{tabular}      & No                                                                       & Yes                                                                      & No                                                                       & Yes                                                                      \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
                                                                                      &                                                                          &                                                                          &                                                                          &                                                                          \\ \hline
Observations                                                                          & 143,105                                                                  & 143,105                                                                  & 56,346                                                                   & 56,346                                                                   \\ \hline
R-squared                                                                             & 0.296                                                                    & 0.377                                                                    & 0.001                                                                    & 0.121                                                                    \\ \hline
\multicolumn{5}{|l|}{Robust standard errors in parentheses}                                                                                                                                                                                                                                                                                                                                       \\ \hline
\multicolumn{5}{|l|}{*** p\textless0.01, ** p\textless0.05, * p\textless0.1}                                                                                                                                                                                                                                                                                                                      \\ \hline
\end{tabular}
\end{table}

==> plots/persistence-regs.tex <==

% Table created by stargazer v.5.2 by Marek Hlavac, Harvard University. E-mail: hlavac at fas.harvard.edu
% Date and time: Sun, Jan 06, 2019 - 12:32:33 AM
\begin{table}[!htbp] \centering 
  \caption{} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{\textit{Dependent variable:}} \\ 
\cline{2-3} 
\\[-1.8ex] & trip\_distance\_resid\_3.mean.y.LGA & trip\_distance\_resid\_5.mean.y.LGA \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 trip\_distance\_resid\_3.mean.x.LGA & 0.761$^{***}$ &  \\ 
  & (0.008) &  \\ 
  & & \\ 
 trip\_distance\_resid\_5.mean.x.LGA &  & 0.703$^{***}$ \\ 
  &  & (0.008) \\ 
  & & \\ 
 Constant & 0.019$^{***}$ & 0.120$^{***}$ \\ 
  & (0.006) & (0.008) \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 6,822 & 6,822 \\ 
R$^{2}$ & 0.579 & 0.502 \\ 
Adjusted R$^{2}$ & 0.579 & 0.502 \\ 
Residual Std. Error (df = 6820) & 0.517 & 0.557 \\ 
F Statistic (df = 1; 6820) & 9,382.717$^{***}$ & 6,871.241$^{***}$ \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> plots/persistence-tables.tex <==


\textbf{Same Airport}

\begin{table}[H]
\centering
\caption{LaGuardia Random Split}
\label{persistence-tables}
\begin{tabular}{|c|c|c|}
\hline
                     & First 50\% of Trips & Second 50\% of Trips \\ \hline
First 50\% of Trips  & 1                   & 0.84                 \\ \hline
Second 50\% of Trips & 0.84                & 1                    \\ \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{JFK Random Split}
\label{my-label}
\begin{tabular}{|c|c|c|}
\hline
                     & First 50\% of Trips & Second 50\% of Trips \\ \hline
First 50\% of Trips  & 1                   & 0.57                 \\ \hline
Second 50\% of Trips & 0.57                & 1                    \\ \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{LaGuardia Calendar Split}
\label{my-label}
\begin{tabular}{|c|c|c|}
\hline
                     & First 50\% of Trips & Second 50\% of Trips \\ \hline
First 50\% of Trips  & 1                   & 0.80                 \\ \hline
Second 50\% of Trips & 0.80                & 1                    \\ \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{JFK Calendar Split}
\label{my-label}
\begin{tabular}{|c|c|c|}
\hline
                     & First 50\% of Trips & Second 50\% of Trips \\ \hline
First 50\% of Trips  & 1                   & 0.55                 \\ \hline
Second 50\% of Trips & 0.55                & 1                    \\ \hline
\end{tabular}
\end{table}

\textbf{Cross-Airport}

\begin{table}[H]
\centering
\caption{Cross-Airport Random Split}
\label{my-label}
\begin{tabular}{|c|c|c|}
\hline
                         & JFK First 50\% of Trips & JFK Second 50\% of Trips \\ \hline
LGA First 50\% of Trips  & 0.04                    & 0.05                     \\ \hline
LGA Second 50\% of Trips & 0.02                    & 0.02                     \\ \hline
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{Cross Airport Calendar Split}
\label{my-label}
\begin{tabular}{|c|c|c|}
\hline
                   & JFK Jan-Jun Trips & JFK July-Dec Trips \\ \hline
LGA Jan-Jun Trips  & 0.04              & 0.05               \\ \hline
LGA July-Dec Trips & 0.02              & 0.02               \\ \hline
\end{tabular}
\end{table}

The tables report the correlations between various subsamples according to the methodology in section 6. “Random Split” refers to randomly splitting the sample in half. “January-June vs. July-December Split” refers to splitting the data into two sets: one set being of trips between January 2013 and June 2013, and another set being trips between July 2013 and December 2013. “Cross-Airport” refers to comparisons of correlations between LaGuardia airport and JFK airport.
